Conical resolutions and cohomology of the moduli spaces of nodal hypersurfaces

A projective hypersurface is nodal if it does not have singularities worse than simple nodes. We calculate the rational cohomology of the spaces of equations of nodal cubic and quartic plane curves and also nodal cubic surfaces in the projective 3-space. We deduce the cohomology of the corresponding spaces of equations and moduli spaces. In the case of plane cubics we use the method of conical resolutions. We handle plane quartics by applying a more general version of this method which we construct in this paper. For cubic surfaces we use an explicit description of the compact GIT quotient.

==> singular_input.tex <==
ring r = 0,(e0,e1,e2),dp; //r is the polynomial ring over Q in e1,e2,e3; degree reverse lex ordering.
ideal I=e0+e1+e2,e0*e1+e0*e2+e1*e2,e0*e1*e2; //I is the ideal generated by symmetric polynomials.

//plane nodal cubics
reduce(e1-e2,groebner(I));//Check whether top degree d^1 from 2nd column to 1st is non-zero
reduce(e0*(e1-e2),groebner(I));//Check whether middle degree d^1 from 2nd column to 1st is non-zero
reduce(e0^2*(e1-e2),groebner(I));//Check whether bottom degree d^1 from 2nd column to 1st is non-zero
//now we want to check whether e0*(e1-e2) and (e1-e2)*(-e1-2*e2) are linearly dependent over Q in the
//quotient ring r/I. To this end, we add e0*(e1-e2) to the ideal I, get a new ideal J and reduce 
//(e1-e2)*(-e1-2*e2) mod J. The result is non-zero.
ideal J=I,e0*(e1-e2);
reduce((e1-e2)*(-e1-2*e2),groebner(J));
ideal J1=I,e0;
reduce(e2,groebner(J1)); //Check that e0, e2 are linearly independent mod I (needed for column 6; obvious)
ideal J2=I,e0^2;
reduce(e2^2,groebner(J2)); //Check that e0^2, e2^2 are linearly independent mod I (needed for column 6)

//plane nodal quartics
reduce(e1,groebner(I));//Check whether top degree d^1 from 2nd column to 1st is non-zero
reduce(e0*e1,groebner(I));//Check whether middle degree d^1 from 2nd column to 1st is non-zero
reduce(e0^2*e1,groebner(I));//Check whether bottom degree d^1 from 2nd column to 1st is non-zero

reduce(e0-e2,groebner(I));//d from 6 col: check whether the anti-symmetric element we times by e is non-zero
reduce(2*e1*(e0-e2),groebner(I));//Check whether top degree d^1 from 6th column to 1st is non-zero
reduce(2*e1^2*(e0-e2),groebner(I));//Check whether bottom degree d^1 from 6th column to 1st is non-zero

//plane stable quartics

reduce(e0*e1^2,groebner(I)); // stable quartics

reduce(e1,groebner(I));
reduce(e2,groebner(I,e1));
reduce(e1^2,groebner(I));
reduce(e2^2,groebner(I,e1^2));
reduce(e1^3,groebner(I)); // result = 0
reduce(e0*e1*e2,groebner(I)); // sanity check
reduce(e1*e2^2,groebner(I));
